Applications of Chern-Simons Ward Identities to log(T\tau) Conductivity Calculations of the nu=1/2 System

We reconsider the theory of the half-filled Landau level with impurities using the Chern-Simons formulation and study Ward identities for the Chern-Simons theory. From these we get conductivity diagrams with impurities which obey the continuity equation. We calculate the conductivity of these diagrams for which we obtain log(T\tau) divergent conductivity diagrams for low temperature T. We compare our result with the experimental values of the low temperature conductivities. Finally we calculate the conductivity for small deviations of the magnetic field B from the value nu=1/2. In this case we get a singularity in the conductivity.

==> pst-feyn.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% -*- Mode: Latex -*- %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% pst-feyn.tex --- Generation of feynman diagrams with PSTricks
%%
%% Author          : Thomas SIEGEL <siegel@aix550.informatik.uni-leipzig.de>
%% Created the     : Mon Aug 25 16:02:02 MET DST 1997
%% Last mod. by    : Thomas SIEGEL <siegel@aix550.informatik.uni-leipzig.de>
%% Last mod. the   : Thu Feb 19 17:11:38 MET 1998
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\fileversion{0.94}
\def\filedate{1998/02/19}

\message{`PST-Feynman' v\fileversion , \filedate\space (Thomas Siegel)}

\csname PSTFeynmanLoaded\endcsname
\let\PSTFeynmanLoaded\endinput

% Require PSTricks and pst-plot packages
\ifx\PSTricksLoaded\endinput\else\input pstricks.tex\fi
\ifx\PSTplotLoaded\endinput\else\input pst-plot.tex\fi
\ifx\PSTnodeLoaded\endinput\else\input pst-node.tex\fi

% DPC interface to the KeyVal package (until keyval based version of PSTricks)
\input pst-key.tex

\edef\PstAtCode{\the\catcode`\@}
\catcode`\@=11\relax

% Some macro definitions:
% -----------------------

% Denis Girou addition begin - Dec. 18, 1997

% Adapted from \psset@arrows
\def\psset@ArrowInside#1{%
\begingroup
\pst@activearrows
\xdef\pst@tempg{<#1}%
\endgroup
\expandafter\psset@@ArrowInside\pst@tempg\@empty-\@empty\@nil
\if@pst\else
\@pstrickserr{Bad intermediate arrow specification: #1}\@ehpa
\fi}

% Adapted from \psset@@arrows
\def\psset@@ArrowInside#1-#2\@empty#3\@nil{%
\@psttrue
\def\next##1,#1-##2,##3\@nil{\def\pst@tempg{##2}}%
\expandafter\next\pst@arrowtable,#1-#1,\@nil
\@ifundefined{psas@#2}%
{\@pstfalse\def\psk@ArrowInside{}}%
{\def\psk@ArrowInside{#2}}}
\def\psk@ArrowInside{}


% Modified version of \pst@addarrowdef
\def\pst@addarrowdef{%
\addto@pscode{%
/ArrowA {
\ifx\psk@arrowA\@empty
\pst@oplineto
\else
\pst@arrowdef{A}
moveto
\fi
} def
/ArrowB {
\ifx\psk@arrowB\@empty \else \pst@arrowdef{B} \fi
} def
% DG addition
/ArrowInside {\ifx\psk@ArrowInside\@empty \else \pst@arrowdefA{Inside} \fi} def
}}

% Adapted from \pst@arrowdef
\def\pst@arrowdefA#1{%
\ifnum\pst@repeatarrowsflag>\z@
/Arrow#1c [ 6 2 roll ] cvx def Arrow#1c
\fi
\tx@BeginArrow
\psk@arrowscale
\@nameuse{psas@\@nameuse{psk@Arrow#1}}
\tx@EndArrow}

% ArrowInsidePos parameter
\def\psset@ArrowInsidePos#1{\pst@checknum{#1}\psk@ArrowInsidePos}%
\psset@ArrowInsidePos{0.5}

% ArrowAdjust parameter
% T.S.  addition begin 
\newif\ifPst@ArrowAdjust
\define@key{psset}{ArrowAdjust}[false]{%
\@nameuse{Pst@ArrowAdjust#1}}
% T.S.  addition end

% T.S.  addition begin
\def\pst@ArrowScaleX{1 }%
\def\pst@ArrowScaleY{1 }%
% T.S.  addition end

% Modified version of \pst@getscale
\def\pst@getscale#1#2{%
\pst@expandafter\pst@getnumii{#1 #1} {} {} {}\@nil
\@psttrue
\ifdim\pst@tempg\p@=\z@
\@pstrickserr{Bad scaling argument #1'}\@ehpa
\def\pst@tempg{1 }%
\@pstfalse
\fi
\ifdim\pst@temph\p@=\z@
\if@pst\@pstrickserr{Bad scaling argument #1'}\@ehpa\fi
\def\pst@temph{1 }%
\fi
% T.S.  addition begin
\edef\pst@ArrowScaleX{\pst@tempg}%
\edef\pst@ArrowScaleY{\pst@temph}%
% T.S.  addition end
\edef#2{\pst@tempg\space \pst@temph\space scale }%
\ifdim\pst@tempg\p@=\p@ \ifdim\pst@temph\p@=\p@
\def#2{}%
\fi\fi}



% Redefinition of the PostScript /Line macro to print the intermediate arrow
% on each segment of the line
\pst@def{Line}<{%
NArray
n 0 eq not
  { n 1 eq { 0 0 /n 2 def } if
    2 copy
    /y1 ED
    /x1 ED
    ArrowA
    x1 y1
    /n n 1 sub def
    n { 4 copy
        /y1 ED
        /x1 ED
        /y2 ED
        /x2 ED
% T.S.  addition begin
        /dx x2 x1 sub def
        /dy y2 y1 sub def
        \ifPst@ArrowAdjust
         /@arrowwidth
           \psk@arrowsize
           \pst@number\pslinewidth mul
           add
         def
         /@arrowlength             
           \psk@arrowlength 
           @arrowwidth mul \pst@ArrowScaleY\space mul
         def
         \ifx\pslinestyle\@none
           /@adjustment 0 def
         \else
          /@adjustment
            \pst@number\pslinewidth 
            @arrowlength mul 
            @arrowwidth \pst@ArrowScaleX\space mul div
          def
         \fi
         /@arrowlength 
           @arrowlength 
           @adjustment add 
         def
         /t              % ÄßredßmyboxÄ$t=ßfracÄ@arrowlengthÜÄ2ßsqrtÄdx^2 + dy^2ÜÜ$ÜÜ
           @arrowlength
           dx dx mul dy dy mul add 
           sqrt 2 mul 
           div 
         def
        \else
         /t 0 def
        \fi
        /aposx dx \psk@ArrowInsidePos t add mul x1 add def
        /aposy dy \psk@ArrowInsidePos t add mul y1 add def
        x1 y1 aposx aposy ArrowInside pop pop pop pop Lineto
% T.S.  addition end
      } repeat
    CP 4 2 roll ArrowB L pop pop } if}>

% Denis Girou addition end


%
% common variables for \WavyLine and \WavyArc :
%

\define@key{psset}{A}{%   
\edef\psk@A{#1}}

\define@key{psset}{n}{%
\edef\psk@n{#1}}

\define@key{psset}{alpha}{%
\edef\psk@alpha{#1}}

\define@key{psset}{beta}{%
\edef\psk@beta{#1}}

\def\WavyLine{\pst@object{WavyLine}}%

\def\WavyLine@i{%
\setkeys{psset}{plotpoints=200,
                alpha=0,beta=0,
                A=.1,n=10}%
\begin@OpenObj
\pst@getcoors[\WavyLine@ii}
\def\WavyLine@ii{%
\addto@pscode{\WavyLine@iii}%
\showpointsfalse
\end@OpenObj}

\def\WavyLine@iii{%
/CoorField 4 array def
CoorField astore pop
/x1 { CoorField 2 get }  def
/y1 { CoorField 3 get }  def
/x2 { CoorField 0 get }  def
/y2 { CoorField 1 get }  def
/hypot { x2 x1 sub dup mul y2 y1 sub dup mul add sqrt }  def
/ep { \psk@n\space 2 mul hypot mul }  def
/bn { ep 360 div round 360 mul \psk@beta\space add }  def
/korr { bn \psk@alpha\space sub ep div }  def
/Shape {
  2 hypot mul korr mul t mul \psk@n\space mul 
  \psk@alpha\space add sin \psk@A\space mul \pst@number\psunit mul 
  } 
def
/denome { Shape hypot div }  def
/xOrtho { y2 y1 sub denome mul }  def
/yOrtho { x2 x1 sub denome mul }  def
/step { 1 \psk@plotpoints\space div }  def
/i 0 def
\psk@plotpoints 1 add {
    /t i step mul def 
    /i i 1 add def
    x2 x1 sub t mul
    x1 add
    xOrtho sub
    y2 y1 sub t mul
    y1 add
    yOrtho add
    t 0 eq { moveto } { lineto } ifelse
} repeat }


\def\WavyArc{\pst@object{WavyArc}}

\def\WavyArc@i{%
\setkeys{psset}{plotpoints=400,
                alpha=0,beta=0,
                A=.1,n=10}%
\@ifnextchar({\WavyArc@ii}{\WavyArc@ii(0,0)}}

\def\WavyArc@ii(#1)#2#3#4{%
\begin@OpenObj
\pst@getangle{#3}\pst@tempa
\pst@getangle{#4}\pst@tempb
\pst@@getcoor{#1}%
\edef\@Radius{#2 \pst@number\psunit mul \space}%
\addto@pscode{\WavyArc@iii}%
\showpointsfalse
\end@OpenObj}

\def\WavyArc@iii{%
\pst@coor
/CoorField 2 array def
CoorField astore pop
/x1 { CoorField 0 get }  def
/y1 { CoorField 1 get }  def
/r \@Radius def
/c 57.2957 r \tx@Div def
/angleA \pst@tempa def
/angleB \pst@tempb def
angleA angleB gt { /angleB angleB 360 add def } if
/n { \psk@n\space \pst@number\psunit div }  def
/A { \psk@A\space \pst@number\psunit mul }  def
/dp { angleB angleA sub }  def
/a { angleA n mul r mul }  def
/b { dp n mul r mul a add }  def
/an {
  a 360 div round 360 mul \psk@alpha\space
  add n r mul div } 
def
/bn {
  b 360 div round 360 mul \psk@beta\space
  add n r mul div } 
def
/dpn { bn an sub }  def
/arg { dpn t mul an add n mul r mul }  def
/T { dp t mul angleA add }  def
/step { 1 \psk@plotpoints\space div }  def
/i 0 def
\psk@plotpoints 1 add {
    /t i step mul def
    /i i 1 add def
    T cos arg sin A mul r add mul x1 add
    T sin arg sin A mul r add mul y1 add
    t 0 eq { moveto } { lineto } ifelse
} repeat }


\newif\ifPst@turn
\define@key{psset}{turn}[false]{%
\@nameuse{Pst@turn#1}}

\def\Photon{%
\@ifnextchar[\@Photon{\@Photon[]}}

\def\@Photon[#1](#2)(#3)#4{%
\setkeys{psset}{turn=false}%
\setkeys{psset}{#1}%
\SpecialCoor%
\pnode(#2){PhotonBegin}%
\pnode(#3){PhotonEnd}%
\pnode(0,0){Origin}%
\psline(PhotonBegin)(PhotonEnd)%
\nc@object{Open}{PhotonBegin}{PhotonEnd}{.5}{%
tx@Dict begin 
/@xA xA def
/@yA yA def
/@xB xB def
/@yB yB def
/@r #4 def
end}
\nc@object{Open}{Origin}{PhotonBegin}{.5}{%
tx@Dict begin 
/@ox xB xA sub def
/@oy yB yA sub def
end}
\ifPst@turn
\rput(!@xB @xA sub 2 div \pst@number\psxunit div @ox \pst@number\psxunit div add
@yB @yA sub 2 div \pst@number\psyunit div @oy \pst@number\psyunit div add){%
\WavyArc[beta=180,#1]
{@xB @xA sub dup mul @yB @yA sub dup mul add sqrt 
2 div @r mul \pst@number\psunit div}%
{(PhotonBegin)}{(PhotonEnd)}}
\else
\rput(!@xB @xA sub 2 div \pst@number\psxunit div @ox \pst@number\psxunit div add
@yB @yA sub 2 div \pst@number\psyunit div @oy \pst@number\psyunit div add){%
\WavyArc[beta=180,#1]
{@xB @xA sub dup mul @yB @yA sub dup mul add sqrt 
2 div @r mul \pst@number\psunit div}%
{(PhotonEnd)}{(PhotonBegin)}}
\fi
}



%
% common variables for \CycloidLine, \EpiCycloid 
% and HypoCycloid :
%

\newif\ifadaption
\def\psset@adaption#1{\@nameuse{adaption#1}}
\psset@adaption{true}

\define@key{psset}{r}{%
\edef\psk@r{#1}}

\define@key{psset}{a}{%
\edef\psk@a{#1}}

\def\CycloidLine{\pst@object{CycloidLine}}%

\def\CycloidLine@i{%
\setkeys{psset}{plotpoints=200,
                r=0.05,a=0.15}%
\begin@OpenObj
\pst@getcoors[\CycloidLine@ii}
\def\CycloidLine@ii{%
\addto@pscode{\CycloidLine@iii}%
\ifadaption
\addto@pscode{\CycloidLine@iv}%
\else
\addto@pscode{\CycloidLine@v}%
\fi
\addto@pscode{\CycloidLine@vi}%
\showpointsfalse
\end@OpenObj}

\def\CycloidLine@iii{%
/CoorField 4 array def
CoorField astore pop
/x1 { CoorField 2 get } def
/y1 { CoorField 3 get } def
/x2 { CoorField 0 get } def
/y2 { CoorField 1 get } def
/pipi 6.283185307179586477 def
/Sin { 360 mul pipi div sin } def
/Cos { 360 mul pipi div cos } def
/hypot { x2 x1 sub dup mul y2 y1 sub dup mul add sqrt } def
/Radius { \psk@r\space \pst@number\psunit mul } def
/Amplitude { \psk@a\space \pst@number\psunit mul } def
/fkt_x { dup Radius mul exch Sin Amplitude  mul sub } def
/fkt_y { Cos Amplitude  mul Radius exch sub } def
}

\def\CycloidLine@iv{%
 /newton { % define newton iteration to solve a diophantic equation:
   dup dup dup
   Sin Amplitude mul exch Radius mul sub exch
   Cos Amplitude mul Radius sub div sub
 } def
 /start
  1 1 15 { % 15 should be enough ...
   1 eq {
    1 Radius Amplitude div sub 6 mul sqrt
   } if
   newton
  } for
 def
 /offset start fkt_y def
 /n hypot pipi Radius mul div round def
 /f hypot n pipi mul Radius mul div 1 mul def
}

\def\CycloidLine@v{%
 /start 0 def
 /offset 0 def
 /n hypot pipi Radius mul div def
 /f 1 def
} 

\def\CycloidLine@vi{%
x1 y1 translate % assume the centimeter mode
y2 y1 sub x2 x1 sub atan rotate
/ende n pipi mul start sub def 
/step ende start sub \psk@plotpoints\space div def
/i 0 def
 \psk@plotpoints 1 add {
    /t start i step mul add def
    /i i 1 add def
    t fkt_x f mul
    t fkt_y offset sub
    t start eq { moveto } { lineto } ifelse
 } repeat 
}


\def\EpiCycloid{\pst@object{EpiCycloid}}%

\def\EpiCycloid@i{%
\setkeys{psset}{plotpoints=300,
                r=.05,a=.15}%
\@ifnextchar({\EpiCycloid@ii}{\EpiCycloid@ii(0,0)}}

\def\EpiCycloid@ii(#1)#2#3#4{%
\begin@OpenObj
\pst@@getcoor{#1}%
\pst@getangle{#3}\pst@tempa
\pst@getangle{#4}\pst@tempb
\edef\@Radius{#2 \pst@number\psunit mul \space}%
\addto@pscode{\EpiCycloid@iii}%
\ifadaption
\addto@pscode{\EpiCycloid@iv}%
\else
\addto@pscode{\EpiCycloid@v}%
\fi
\addto@pscode{\EpiCycloid@vi}%
\ifadaption
\addto@pscode{\EpiCycloid@vii}%
\else
\addto@pscode{\EpiCycloid@viii}%
\fi
\addto@pscode{\EpiCycloid@ix}%
\ifadaption
\addto@pscode{\EpiCycloid@x}%
\else
\addto@pscode{\EpiCycloid@xi}%
\fi
\addto@pscode{\EpiCycloid@xii}%
\showpointsfalse
\end@OpenObj}


\def\EpiCycloid@iii{%
\pst@coor
/CoorField 2 array def
CoorField astore pop
/x1 { CoorField 0 get } def
/y1 { CoorField 1 get } def
/angleA \pst@tempa def
/angleB \pst@tempb def
angleA angleB gt { /angleB angleB 360 add def } if
/r {\psk@r\space \pst@number\psunit mul}  def
/a {\psk@a\space \pst@number\psunit mul}  def
/pipi 6.283185307179586477 def % ßred$2ßpi$
/end angleB angleA sub pipi mul 360 div def % ßred$ÄßscriptstyleßfracÄ2ßpi(ßbeta-ßalpha)ÜÄ360ÜÜ$
/Sin { 360 mul pipi div sin } def % ßred$ßsinÄßscriptstyleßfracÄ360ÄÜtÜÄ2ßpiÜÜ$
/Cos { 360 mul pipi div cos } def % ßred$ßcosÄßscriptstyleßfracÄ360ÄÜtÜÄ2ßpiÜÜ$
}

\def\EpiCycloid@iv{%
/f
  \@Radius end mul pipi r mul
  div round pipi mul r mul
  end \@Radius mul div % ßredßmyboxÄ$f=ßfracÄ2ßpiÄÜrÜÄRßcdotßmboxÄendÜÜßcdotßmboxÄRoundÜßleft(ßfracÄRßcdotßmboxÄendÜÜÄ2ßpiÄÜrÜßright)$Ü
def
} 

\def\EpiCycloid@v{/f 1 def} % ßred$f=1$

\def\EpiCycloid@vi{
/fkt_x { dup Cos \@Radius r add mul
         exch \@Radius r div f mul 1
         add mul Cos a mul sub } def
/fkt_y { dup Sin \@Radius r add mul
         exch \@Radius r div f mul 1
         add mul Sin a mul sub } def
x1 y1 translate
}

\def\EpiCycloid@vii{angleA}

\def\EpiCycloid@viii{0}

\def\EpiCycloid@ix{
rotate
/newton {     % ßredßtextitÄdefine newton iteration to solve aÜ
  dup dup dup % ßredßtextitÄdiophantic equation:Ü
  Sin r \@Radius add mul exch f \@Radius mul
  r div 1 add mul Sin a mul sub
  exch dup
  Cos r \@Radius add mul exch f \@Radius mul
  r div 1 add mul Cos a mul
  f \@Radius mul r div 1 add mul sub div sub
} def
}

\def\EpiCycloid@x{
/start
  1 1 15 { % ßredßtextitÄ15 should be enough ...Ü
   1 eq {
    r \@Radius add r mul f \@Radius mul
    r add a mul sub
    r dup mul mul
    r \@Radius add r dup dup mul mul mul
    f \@Radius mul r add dup dup mul mul
    a mul sub div
    6 mul sqrt
   } if
   newton
  } for
def
}

\def\EpiCycloid@xi{/start 0 def}

\def\EpiCycloid@xii{
/step { 
  end start sub 
  start sub 
  \psk@plotpoints\space div 
} def
/i 0 def
\psk@plotpoints 1 add {
    /t start i step mul add def
    /i i 1 add def
    t fkt_x
    t fkt_y
    t start eq { moveto } { lineto } ifelse
} repeat }


\newif\ifadaption
\def\psset@adaption#1{\@nameuse{adaption#1}}
\psset@adaption{true}

\define@key{psset}{r}{%
\edef\psk@r{#1}}

\define@key{psset}{a}{%
\edef\psk@a{#1}}



\def\HypoCycloid{\pst@object{HypoCycloid}}%

\def\HypoCycloid@i{%
\setkeys{psset}{plotpoints=300,
                r=.05,a=.15}%
\@ifnextchar({\HypoCycloid@ii}{\HypoCycloid@ii(0,0)}}

\def\HypoCycloid@ii(#1)#2#3#4{%
\begin@OpenObj
\pst@@getcoor{#1}%
\edef\@Radius{#2 \pst@number\psunit mul \space}%
\pst@getangle{#3}\pst@tempa
\pst@getangle{#4}\pst@tempb
\addto@pscode{\HypoCycloid@iii}%
\ifadaption
\addto@pscode{\HypoCycloid@iv}%
\else
\addto@pscode{\HypoCycloid@v}%
\fi
\addto@pscode{\HypoCycloid@vi}%
\ifadaption
\addto@pscode{\HypoCycloid@vii}%
\else
\addto@pscode{\HypoCycloid@viii}%
\fi
\addto@pscode{\HypoCycloid@ix}%
\ifadaption
\addto@pscode{\HypoCycloid@x}%
\else
\addto@pscode{\HypoCycloid@xi}%
\fi
\addto@pscode{\HypoCycloid@xii}%
\showpointsfalse
\end@OpenObj}


\def\HypoCycloid@iii{%
\pst@coor
/CoorField 2 array def
CoorField astore pop
/x1 { CoorField 0 get } def
/y1 { CoorField 1 get } def
/angleA \pst@tempa def
/angleB \pst@tempb def
angleA angleB gt { /angleB angleB 360 add def } if
/r {\psk@r\space \pst@number\psunit mul}  def
/a {\psk@a\space \pst@number\psunit mul}  def
/pipi 6.283185307179586477 def
/end angleB angleA sub pipi mul 360 div def
/Sin { 360 mul pipi div sin } def
/Cos { 360 mul pipi div cos } def
}

\def\HypoCycloid@iv{%
/f
  \@Radius end mul pipi r mul 
  div round pipi mul r mul 
  end \@Radius mul div
def
} 

\def\HypoCycloid@v{/f 1 def}

\def\HypoCycloid@vi{
/fkt_x { dup Cos \@Radius r sub mul 
         exch \@Radius r div f mul 1
         sub mul Cos a mul add } def
/fkt_y { dup Sin \@Radius r sub mul 
         exch \@Radius r div f mul 1
         sub mul Sin a mul sub } def
x1 y1 translate
}

\def\HypoCycloid@vii{angleA}

\def\HypoCycloid@viii{0}

\def\HypoCycloid@ix{
rotate
/newton { % define newton iteration to solve a diophantic equation:
   dup dup dup
   Sin \@Radius r sub mul exch f \@Radius mul 
   r div 1 sub mul Sin a mul sub
   exch dup
   Cos \@Radius r sub mul exch f \@Radius mul 
   r div 1 sub mul Cos a mul 
   f \@Radius mul r div 1 sub mul sub div sub
} def
}

\def\HypoCycloid@x{
/start
  1 1 15 { % 15 should be enough ...
   1 eq {
    r \@Radius sub 1 f \@Radius mul 
    r div sub a mul sub
    r \@Radius sub 6 div f \@Radius mul 
    r div 1 sub dup dup mul mul 
    a mul 6 div add
    div sqrt
   } if
   newton
  } for
def
}

\def\HypoCycloid@xi{/start 0 def}

\def\HypoCycloid@xii{
/step { 
  end start sub 
  start sub 
  \psk@plotpoints\space div 
} def
/i 0 def
\psk@plotpoints 1 add {
    /t start i step mul add def
    /i i 1 add def
    t fkt_x
    t fkt_y
    t start eq { moveto } { lineto } ifelse
} repeat }

\catcode`\@=\PstAtCode\relax
\endinput
%%
%% END: pst-feyn.tex

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pst-key.tex "
%%% End: 


==> pst-key.tex <==
%%
%% This is file `pst-key.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% keyval.dtx  (with options: `package,plain,pstricks')
%% 
%% This file is based on keyval.dtx from the LaTeX tools distribution.
%% It may be distributed and used with the conditions applying to the
%% PSTricks distribution. See the comments in pstricks.tex for details.
%% 
%% File: keyval.dtx Copyright (C) 1993 1994 1995 1997 David Carlisle
\def\next[#1]{\catcode`\@=11
       \expandafter\let\csname ver@keyval.sty\endcsname\empty
       \wlog{keyval: #1}}\next
                 [1997/06/13 v1.10 key=value parser (DPC)]
\def\setkeys{%
  \@ifnextchar[%
    \KV@list
    {\let\KV@undefined\KV@error
     \KV@setkeys}}
\def\KV@psset{psset}
\def\KV@setkeys#1#2{%
  \def\@tempa{#1}%
  \edef\KV@prefix{%
  \ifx\@tempa\KV@psset\else
                  KV@%
  \fi
                  #1@}%
  \KV@do#2,\relax,}
\def\psset#1{%
  \def\KV@prefix{psset@}%
  \KV@do#1,\relax,}
\def\use@par{\expandafter\psset\expandafter{\pst@par}}
\def\KV@list[#1]{%
  \def\KV@undefined{\KV@add#1}%
   \ifx#1\@undefined
    \let#1\@empty
   \fi
  \KV@setkeys}
\def\KV@do#1,{%
 \ifx\relax#1\empty\else
  \KV@split#1==\relax
  \expandafter\KV@do\fi}
\def\KV@split#1=#2=#3\relax{%
  \KV@@sp@def\@tempa{#1}%
  \ifx\@tempa\@empty\else
    \expandafter\let\expandafter\@tempc
      \csname\KV@prefix\@tempa\endcsname
    \ifx\@tempc\relax
      \KV@undefined{#2}{#3}%
    \else
      \ifx\@empty#3\@empty
        \KV@default
      \else
        \KV@@sp@def\@tempb{#2}%
        \expandafter\@tempc\expandafter{\@tempb}\relax
      \fi
    \fi
  \fi}
\def\KV@default{%
  \expandafter\let\expandafter\@tempb
    \csname\KV@prefix\@tempa @default\endcsname
  \ifx\@tempb\relax
    \KV@err{No value specified for \@tempa}%
  \else
    \@tempb\relax
  \fi}
\def\KV@add#1#2#3{%
  \toks2\expandafter{#1}%
  \KV@@sp@def\@tempb{#2}%
  \toks4\expandafter{\@tempb}%
  \edef#1{\the\toks2
          \ifx#1\@empty\else,\fi
          \@tempa
          \ifx\KV@add#3\KV@add\else={\the\toks4}\fi}}
\def\KV@err#1{\errmessage{keyval: #1}}
\def\KV@error#1#2{\KV@err{\@tempa\space undefined}}
\def\@tempa#1{%
\def\KV@@sp@def##1##2{\KV@@sp@b##2\@nil\@nil#1\@nil\relax##1}}
\@tempa{ }
\def\KV@@sp@b#1#2 \@nil{\KV@@sp@c#1#2}
\def\KV@@sp@c#1\@nil#2\relax#3{\def#3{#1}}
\def\define@key#1#2{%
  \def\KV@prefix{#1}%
  \edef\KV@prefix{%
    \ifx\KV@prefix\KV@psset\else
        KV@%
     \fi
        #1@#2}%
  \@ifnextchar[\KV@def{\@namedef\KV@prefix####1}}
\def\KV@def[#1]{%
  \@namedef{\KV@prefix @default\expandafter}\expandafter
    {\csname \KV@prefix\endcsname{#1}}%
  \@namedef\KV@prefix##1}
\endinput
%%
%% End of file `pst-key.tex'.

